A rigorous path-integral formula for quantum-spin dynamics via planar Brownian motion

Adapting ideas of Daubechies and Klauder we derive a continuum path-integral formula for the time evolution generated by a spin Hamiltonian. For this purpose we identify the finite-dimensional spin Hilbert space with the ground-state eigenspace of a suitable Sch\"odinger operator on $L^2({\mathbb{R}}^2)$, the Hilbert space of square-integrable functions on the Euclidean plane ${\mathbb{R}}^2$, and employ the Feynman-Kac-It\^o formula.

==> definitionen.tex <==
\RequirePackage{amsbsy}

%
%e-Funktion
\newcommand\ep[1]{{e}^{\,\mbox{\small $ #1 $}}}
%
%one (unity)
\newcommand\one{\leavevmode\hbox{\small1\kern-3.78pt\normalsize1}}%
%1/2
\newcommand\half{{\frac 12}}

%Wiener
\newcommand{\dmut}{\int  \mkern-6mu d \mu_{z\!,0;z',t}^{(\nu)}(b) \;}
\newcommand{\dmuu}{\int  \mkern-6mu d \mu_{z\!,0;z',u}^{(\nu)}(b) \;}
\newcommand{\Idmut}{d \mu_{z\!,0;z',t}^{(\nu)}(b)}

% Command for Bras. Example: with "\bra{1}" you get "<1|".
\newcommand{\ket}[1]{|\mkern0.2mu\mbox{$#1$}\rangle}  
% \ket{1}: |1>
\newcommand{\bra}[1]{\langle\mbox{$#1$}\mkern0.2mu|}              
\newcommand\braket[2]{\langle#1|#2\rangle}
%
%Dickerpunkt
\newcommand\bcdot{\mbox{\boldmath$\cdot$\unboldmath}}
%
\newcommand\abs[1]{\left\vert {#1}\right\vert}
%
\newcommand{\eq}[1]{(\ref{#1})}
%
\newcommand\norm[1]{{\left\vert\mkern-2mu\left\vert #1 \right\vert\mkern-2mu\right\vert}}

% der Punkt -- works beautifully

\renewcommand\dot[1]{\stackrel{\mkern2mu\mbox{}_{\mbox{\bf .}}}{\raisebox{-0pt}{$#1$}}\mkern-5mu}
